Curriculum-guided Abstractive Summarization for Mental Health Online Posts

Automatically generating short summaries from users' online mental health posts could save counselors' reading time and reduce their fatigue so that they can provide timely responses to those seeking help for improving their mental state. Recent Transformers-based summarization models have presented a promising approach to abstractive summarization. They go beyond sentence selection and extractive strategies to deal with more complicated tasks such as novel word generation and sentence paraphrasing. Nonetheless, these models have a prominent shortcoming; their training strategy is not quite efficient, which restricts the model's performance. In this paper, we include a curriculum learning approach to reweigh the training samples, bringing about an efficient learning procedure. We apply our model on extreme summarization dataset of MentSum posts -- a dataset of mental health related posts from Reddit social media. Compared to the state-of-the-art model, our proposed method makes substantial gains in terms of Rouge and Bertscore evaluation metrics, yielding 3.5% (Rouge-1), 10.4% (Rouge-2), and 4.7% (Rouge-L), 1.5% (Bertscore) relative improvements.

==> SECTIONS/01_intro.tex <==
\section{Introduction}

% Text summarization systems aim to condense a piece of text to a shorter form that preserves the major information within the original text. This task is broadly done in two ways: (1) extractive~\cite{Nallapati2017SummaRuNNerAR, Xiao2019ExtractiveSO, Xu2020DiscourseAwareNE} which assembles the salient sentences directly from the source text, and (2) abstractive~\cite{elikyilmaz2018DeepCA, Lebanoff2018AdaptingTN, Liu2019TextSW, Zou2020PretrainingFA, sotudeh-etal-2021-tldr9} that involves paraphrasing, and generating novel words that are not present in the source text. 
% Recent efforts have also tackled the task using hybrid  models~\cite{See2017GetTT, Hsu2018AUM, Chen2019MultiTaskLF, MacAvaney2019SIG}. 
% By evidence, extractive summarization is less challenging than abstractive~\cite{See2017GetTT,Gehrmann2018BottomUpAS}. This is due to the fact that extractive systems merely \textit{copy} pieces of information from the source. Hence, preserving factuality and grammaticality. On the other hand, abstractive networks rather mimic human behaviour and deal with complex tasks of natural language generation such as paraphrasing, incorporation of external knowledge, and etc.

% Over the last decade, neural summarization models based on RNN~\cite{Hochreiter1997LongSM}, and Transformers~\cite{Vaswani2017Att} have achieved promising results on text summarization. 
% The recent success of pre-trained language models on a wide variety of downstream tasks, including summarization, has driven the current state-of-the-art to a new level. While such approaches generate fluent summaries, 
% in the light of their pre-trained language modeling objectives, 
% they mainly have two drawbacks: 
% (1) selection of salient parts of the source text to be abstractively summaized, and (2) limited training efficiency that hinders generalizing training patterns, and blunting model convergence. 
%  a few studies have recognized \textit{content selection} as their pitfall~\cite{Gehrmann2018BottomUpAS,Narayan2020StepwiseES}, restricting the model performance at generating \textit{informative} summaries. In this research, we aim to extend the decoder by inducing sentential information as a \textit{saliency signal} that can come in handy when summarizing the source. 
%  scattered in the source text
%  as opposed to prior work that explored this possibility by extending the encoder~\cite{Akiyama2021HieBARTDS}.

% A number of recent studies have reported the limited training efficiency of Transformer-based models. To be more specific, 

Summarization of mental health online posts is an emerging task that aims to summarize users' posts who are seeking help to enhance their mental state in online networks such as Reddit~\footnote{\url{https://www.reddit.com/}} and Reachout~\footnote{\url{https://au.reachout.com/}}. The post might address several issues of the user's concerns or simply be an elaboration on the user's mental and emotional situation. With user preference, each user-written post can be accompanied by a succinct summary (known as \tldr~\footnote{\tldr{} is the abbreviation of ``Too Long, Didn't Read''. We use ``\tldr{}'' and ``summary'' exchangeably in this paper.}), condensing major points of the user post. This \tldr{} summary is deemed to urge the counselors for a faster read of the user's posted content before reading the post in its entirety; hence, counsellors can provide responses promptly. Herein, we aim to improve state-of-the-art results reported in \cite*{Sotudeh2022MentSumAR} for this task.

% The task is  defined as generating a succinct summary (a.k.a \tldr~\footnote{We use ``\tldr{}'' and ``summary'' exchangeably in this paper.}) of the user-written content ---that is an elaboration of the user's mental situation--- in high abstraction. 

% From the modeling perspective, this behaviour is mainly due to the model complexity.
% i.e., inclusion of millions of learnable parameters that often are time-consuming and resource exhaustive to be optimally tuned.
Large-scale deep neural models are often hard to train, leaning on intricate heuristic set-ups, which can be time-consuming and expensive to tune~\cite{Gong2019EfficientTO, Chen2021EarlyBERTEB}. This is especially the case for the Transformers-based summarizers, which have been shown to consistently outperform the RNN networks when rigorously tuned~\cite{Popel2018TrainingTF}, but also require heuristics such as specialized learning rates and large-batch training~\cite{Platanios2019CompetencebasedCL}. In this paper, we attempt to overcome the mentioned problem on \bart{}~\cite{Lewis2020BARTDS} Transformers-based summarizer by introducing a \textit{Curriculum Learning (CL)} strategy~\cite{Bengio2009CurriculumL} for training the summarization model, leading to improved convergence time, and performance. 

Inspired by humans' teaching style, \textit{curriculum learning} suggests moving the teaching process from easier samples to more difficult ones and dates back to the nineties~\cite{Elman1993LearningAD}. The driving idea behind this approach is that networks can accomplish better task learning when the training instances are exposed to the network in a specific and certain order, from easier samples to more difficult ones~\cite{Chang2021DoesTO}. In the context of neural networks, this process can be thought of as a technique that makes the network robust to getting stuck at local optima, which is more likely in the early stages of the training process. Given the mentioned challenge of summarization networks, we utilize the \superl~\cite{Castells2020SuperLossAG} function that falls into the family of confidence-aware curriculum learning techniques, introducing a new parameter called confidence (i.e., $\sigma$) to the network. 
% While learning this parameter is inefficient, \superl{} bridges by directly using the converged value of confidence at a specific learning state. 
We validate our model on \mentsum~\cite*{Sotudeh2022MentSumAR} dataset,  containing over 24k instances mined from 43 mental health related communities on Reddit social media. Our experimental results show the efficacy of applying curriculum learning objectives on \bart{} summarizer, achieving a new state-of-the-art performance. 
% To measure our model's cross-domain performance, we further report model performance on CNN/DM~\cite{See2017GetTT} and XSum~\cite{Narayan2018DontGM} large-scale news datasets.
% We show that the inclusion of curriculum learning allows for a remarkable performance of neural Transformer-based summarizers.

% While learning this parameter is inefficient, especially on the abundance of training instances such as in summarization, \superl{} bridges this limitation by directly using the converged value of confidence at a specific learning state. 

% CL can be accomplished by assigning a weight to the respective loss, controlling the sample's contribution in learning stage~\cite{Castells2020SuperLossAG}. 

% Systems equipped with curriculum learning have been reported to show strong generalization, faster convergence time, and even improved model performance~\cite{Platanios2019CompetencebasedCL}.

% After identifying the two drawbacks above (i.e., content selection and inefficient training) of Transformer-based networks, we develop our summarization framework to address these shortcomings. 
% To remedy the first drawback, we propose to augment the transformer decoder with a \textit{sentence cross-attention layer}, encouraging the decoder to pay more attention to salient sentences of the source text while generating the abstractive summary.
% Given the aforementioned challenge of the \bart{} as the state-of-the-art abstractive summarizer, we supply the  model with curriculum learning objectives.


% We further carry out a comprehensive human evaluation to examine the efficacy of our model in terms of three qualitative metrics: fluency, informativeness, and overall quality. Our code is made publicly available at [\textit{HTTP}] to facilitate the ongoing research in this direction.

==> SECTIONS/02_related.tex <==
\section{Related Work}
% \begin{figure}[h]
    % \centering
    % \includegraphics[scale=0.3]{LaTeX/samples/figs/BART.pdf}
    % \caption{Caption}
    % \label{fig:my_label}
% \end{figure}
% \textbf{Pre-trained Language Modeling.}
% During the last few years, self-supervised pre-trained language models~\cite{Devlin2019BERTPO, Liu2019RoBERTaAR, Peters2018DeepCW} have gained increased attention from research community due to their considerable improvements in a variety of NLP tasks, including text summarization.
% Different variants of such models are pre-trained on a large amount of unlabeled data, each with various pre-training objectives. 
% While such models are inherently proposed to perform language modeling task, it has been made possible to fine-tune them on a wide range of downstream NLP tasks, summarization being one of them.
% \citet{Liu2019TextSW} were the first to fine-tune \textsc{Bert} for summarization task. 
% They specifically proposed three variants of \textsc{BertSum} including \textsc{BertSumExt} for extractive summarization, \textsc{BertSumAbs} for abstractive summarization, and \textsc{BertSumExtAbs} which is a two-stage fine-tuning approach, exploiting extractive and abstractive objectives. 
% Following up this line of research, ~\citet{zhang2019pegasus} proposed \textsc{Pegasus} with pre-training objectives specific for text summarization and achieved state-of-the-art results on 12 downstream summarization tasks. In a parallel line, \citet{Lewis2020BARTDS} proposed \textsc{Bart} and showed its efficacy on language generation tasks such as text summarization. Unlike \textsc{BertSum} that uses merely pre-trained \textsc{Bert} encoder, \textsc{Pegasus} and \textsc{Bart} exploit both pre-trained encoder and decoder for language generation. 

% \noindent \textbf{Sentence-guided Summarization.}
% Using sentence representations as extractive signals along with token embeddings in neural sequence-to-sequence models has a recent history. This idea is inspired by the fact that while the general encoder-decoder frameworks produce fluent targets, they often fall short in content selection~\cite{Sotudeh2020AttendTM}. A few works have noted that this problem can be addressed by combining extractive and abstractive objectives~\cite{Gehrmann2018BottomUpAS}. While there have been numerous efforts in combining such objectives in traditional RNN networks~\cite{See2017GetTT, Chen2019MultiTaskLF, Lebanoff2018AdaptingTN}, a few studies have explored their efficacy in Transformer-based networks. For instance, \citet{Liu2019TextSW} proposed \textsc{BertSumExtAbs} to utilize extractive objectives from \textsc{BertSumExt} model and further incorporate it with the Transformers decoder to perform abstractive summarization. More recently, \citet{Akiyama2021HieBARTDS} proposed \textsc{Hie-Bart} that adds a self-attention layer for incorporating sentence importance in the encoder. While they augment the encoder with sentential information in the encoder side, the incorporation of such module in the decoder has not been explored in literature. To the best of our knowledge, we are the first to explore this direction on Transformers-based networks in our paper. 

% \noindent \textbf{Curriculum Learning.}
While majority of works in mental health research have focused on studying users' behavioral patterns through classification and prediction tasks~\cite{Choudhury2013PredictingDV,Resnik2013UsingTM,Coppersmith2014MeasuringPT,Yates2017DepressionAS,Cohan2017TriagingCS,Cohan2018SMHDAL,MacAvaney2018RSDDTimeTA}, summarization of online mental health posts has been recently made viable. ~\citet*{Sotudeh2022MentSumAR} were the first to step on this direction via introducing \mentsum dataset of online mental health posts, pinpointing the baseline results.  Curriculum Learning (CL) has gained growing interest from the research communities during the last decade~\cite{Tay2019SimpleAE, MacAvaney2020TrainingCF, Xu2020CurriculumLF}.
% although it has been studied for decades.
% The underlying idea of this technique is to provide a training strategy that flows the learning process from easy samples to the harder ones, which results in improving model performance, decreasing training time, and enhancing the model's generalization ability~\cite{Chang2021DoesTO}. 
\citet{Bengio2015ScheduledSF} were the first to apply this strategy in the context of sequence prediction through \textit{scheduled sampling} approach, which gently changes the training process from ground truth tokens to model-generated ones during decoding. 
% \citet{Platanios2019CompetencebasedCL} proposed a CL-based NMT framework that decides to visit training samples based on their difficulty and competence state of the model.
Sample's \textit{difficulty} is a key concept in this scheme as it is used to distinguish easy examples from difficult ones. Researchers have used many textual features as the ``difficulty measure'' including n-gram frequency~\cite{Haffari2009ActiveLF}, word rarity and sentence length~\cite{Platanios2019CompetencebasedCL}. Recent works~\cite{Saxena2019DataPA, Cachola2020TLDRES} have made use of confidence-aware approaches that learn the difficulty of training samples and dynamically reweight samples in the training process.

==> SECTIONS/03_method.tex <==
% \section{Background}
% \bart~\cite{Lewis2020BARTDS} is a generalized architecture to pre-trained language models based on the Transformer model combining bidirectional and auto-regressive Transformers. \bart is trained by (1) text corruption with an arbitrary noise function; and (2) learning a sequence-to-sequence model to reconstruct the original text. 

% It uses five techniques for pre-training including \textbf{Token masking.} random tokens are masked with \texttt{[MASK]} token similar to \textsc{Bert}~\cite{Devlin2019BERTPO}; \textbf{Token deletion.} deletion of random tokens despite masking them, and the model should decide which positions are missing inputs. \textbf{Text infilling.} inspired by \textsc{SpanBert}~\cite{Joshi2020SpanBERTIP}, a number of text spans are sampled and replaced by \texttt{[MASK]} tokens, and the model learns to predict the number of missing spans; \textbf{Sentence permutation. } sentences in document are randomly shuffled. \textbf{Document rotation. } which teaches the model to predict the start of the document. We refer the reader to the main paper for further explanations. \bart{} has been fine-tuned on a variety of downstream NLP tasks, though it has been shown to be particularly effective when fine-tuned for language generation tasks such as summarization. 
% It uses five techniques for pre-training including \textbf{Token masking.}; \textbf{Token deletion.} \textbf{Text infilling.} inspired by \textsc{SpanBert}~\cite{Joshi2020SpanBERTIP}, a number of text spans are sampled and replaced by \texttt{[MASK]} tokens, and the model learns to predict the number of missing spans; \textbf{Sentence permutation. } sentences in document are randomly shuffled. \textbf{Document rotation. } which teaches the model to predict the start of the document.

% We refer the reader to the main paper for further explanations on pretraining objectives. \bart{} has been fine-tuned on a variety of downstream NLP tasks, though it has been shown to be particularly effective when fine-tuned for language generation tasks such as summarization. 


\section{Our Approach}
In this section, we describe the details of our proposed model, where a curriculum learning architecture is added to the \bart 's Transformers-based framework, upweighting easier training samples; hence, increasing their contribution in learning stage. 
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.27]{FIGS/bart_example.pdf}
%     \caption{\bart's shortcoming in content selection. Yellow: picked by the ground truth, but skipped by \bart{}, Green: picked by both \bart{} and ground truth, and Red: picked by \bart, but skipped by ground truth}
%     \label{fig:bart_shortcoming}
%     \vspace{-0.3cm}
% \end{figure}

% \subsection{Sentence-guided  \textsc{Bart}}
%  As discussed earlier, \bart{} model is one of the well-known pre-trained language modeling approaches that has achieved promising results, being particularly effective for language generation related tasks. 
%  While \bart{} has been shown to be promising in producing abstractive summaries in virtue of its powerful pre-trained encoder and decoder, it suffers from a major pitfall that restricts model efficacy in content selection. Figure \ref{fig:bart_shortcoming} shows a Reddit post along with \bart's generated and ground truth \tldr, demonstrating such a shortcoming. As observed, while the generated summary appears to be well-written and fluent, it ignores salient source regions and focuses on less important parts of the source. Considering the effectiveness of combining extractive and abstractive objectives, we  extend \bart{} by adding a cross-attention layer to induce sentences' importance at decoding time. To this end, we first define a sequence labelling task, where the goal is to predict sentences' \textit{relative importance} score (i.e., $\mathbf{y}$) such that \bart{} is fine-tuned to learn sentential saliency.  The \textit{relative importance} score is casted as the normalized mean of \rgt{} and \rgl{} scores of source sentences with respect to the \tldr{} summary:
% \begin{equation}
    %  \mathbf{y} =    \text{relative importance($s_i$)} = \frac{ \text{RG}_{\text{2+L}}(s_i)}{\sum\limits_{s_i \in R}{\text{RG}_{\text{2+L}}(s_i)}}
    %  \label{eq:importance_score}
% \end{equation}
% where $s_i$ is the sentence in $i$th position, $R$ is the set of post's sentences, and $\text{RG}_{\text{2+L}}(.)$ is a function that takes in a source sentence and outputs the mean of its \rgt{} and \rgl{} scores. For adapting sequence classification task to the sequential sentence tagging problem, we insert \texttt{</s>} tokens (i.e., \texttt{EOS} in \bart{} vocabulary) to the end of each input sentence and then feed it into \bart{} network, similar to \citet{Liu2019TextSW} for \textsc{BertSum}. As \bart{} encodes each input token through its network, the encodings associated with \texttt{</s>} tokens, specifically,  represent input sentences' features preceding them. This is due to the fact that \bart{} uses  \texttt{</s>} tokens' representations as the classification head ~\cite{Lewis2020BARTDS}. After obtaining representations associated with \texttt{</s>} tokens, we process them through a linear layer with Sigmoid classifier to output probabilities as the sentences' importance scores. Formally, let $\mathbf{P}$ be a Reddit post containing sentences $\mathbf{P}=[sent_1, sent_2, ..., sent_i, ..., sent_n]$ and $sent_i=[x_{i1}, x_{i2}, ..., x_{ij}, ..., x_{im}]$.
% where $sent_i$ is the $i$-th sentence within the post and $x_{ij}$ shows the $j$-th word in $sent_i$. 
% We frame input $\mathbf{P}$ by adding \texttt{</s>} tokens to the end, as well as \texttt{<s>} to the start of each sentence. In this sense, the modified input to \bart{} network is $\mathbf{P^\prime} = [\texttt{\textbf{<s>}} sent_1 \footnotesize \texttt{\textbf{</s><s>}} sent_2 ... \footnotesize \texttt{\textbf{</s><s>}} sent_n \footnotesize \texttt{\textbf{</s>}}]$ which is then processed through the \bart{} network. The network is trained to predict the importance score (i.e., $\mathbf{y}$ in Eq \ref{eq:importance_score}). By training such a sequence tagger network, we aim to inject an inductive bias to the \bart{} encoder and decoder to get wised up about the source sentences' importance, which will come in handy when generating abstractive summaries. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.15]{FIGS/Our Model.pdf}
%     \caption{Overview of our summarization model}
%     \label{fig:our_model}
%     \vspace{-0.7em}
% \end{figure}


% At the next stage, we design our framework as demonstrated in Figure \ref{fig:our_model} by extending the decoder with an additional cross-attention layer (i.e., Sentence Multi-Head Attention inside the decoder). We use a two-stage fine-tuning approach to this end, where firstly, we fine-tune the encoder module, as well as the Sentence Multi-head Attention on sequence tagging problem. Second, we further fine-tune it on abstractive summarization task. We separate the optimizers of the pre-trained part (i.e., the encoder and Sentence Multi-Head Attention modules) and the decoder. That is, the pre-trained part should be fine-tuned with a lower learning rate, so it is trained with more accurate gradients as the decoder becomes stable. We name this model as \sentsum{} in our experiments. 


\noindent \textbf{Curricular Learner for \bart{}.}
% Curriculum learning (CL)~\cite{Bengio2009CurriculumL} is a training paradigm to improve the performance and generalization of the learner models based on the idea that easy samples should be visited before the difficult ones during the training~\cite{Castells2020SuperLossAG}. This is due to the fact that when the model starts off with easier samples on early stages of training, the risk of getting stuck in local optima is reduced as most loss functions in deep neural networks are highly non-convex~\cite{Chang2021DoesTO}, and hard to converge. 
Considering the applicability of curriculum learning in training large-scale networks, we aim to use it in our summarization framework. Before incorporating the curriculum learning strategy into our model's training stage, we first need to define the \textit{difficulty} metric to distinguish the hardness of samples. In practice, estimating a prior difficulty for each sample is considered a complex task, so we propose to discriminate the samples with progressive signals ---such as the respective sample loss at each training iteration--- in the training process. In this context, CL is achieved by predicting the difficulty of each sample at the training iterations in the form of a weight, such that difficult samples receive lower weights during the early stages of training and vice versa. To model the curriculum, we propose to use \superl~\cite{Castells2020SuperLossAG} which is a generic loss criterion built upon the task loss function 
as shown in Figure~\ref{fig:superloss}.
\begin{figure}
    \centering
     \includegraphics[scale=0.3]{EMNLP 2022/FIGS/SuperLoss.pdf}
    \caption{Training with standard loss function (left-hand side) and SuperLoss criteria (right-hand side)}. 
    \label{fig:superloss}
    \vspace{-.6em}
\end{figure}

More specifically, \superl{} is a task-agnostic confidence-aware loss function that takes in two parameters: (1) the task loss $\losslrg_i =  \loss(y_i, \widehat{y_i})$, where $y_i$ is neural network's (i.e., \bart's generated summary) output and $\widehat{y_i}$ is the gold label (i.e., ground-truth summary); and (2) $\sigma_i$ as the confidence parameter of the $i$th sample. \superl{} is framed as $\text{L}_{\lambda}(\losslrg_i, \sigma_i)$ and computed as follows,

\begin{equation}
    \text{L}_{\lambda}(\losslrg_i, \sigma_i)= (\losslrg_i - 	\tau) \sigma_i + \lambda (\log \sigma_i)^2
\end{equation}
in which $\lambda$ is the regularization parameter, and $\tau$ is the running or static average of task loss (i.e., $\losslrg$) during the training. While \superl{} provides a well-defined approach to curriculum learning strategy, learning $\sigma$ parameter is not tractable for tasks with abundant training instances such as text summarization. To circumvent this issue and hinder imposing new learnable parameters, \superl{} suggests using the converged value of $\sigma_i$ at the limit,

\begin{align}
\label{eqn:eqlabel}
\begin{split}
\sigma^{*}_{\lambda} (\loss_i) &= \argmin_{\sigma_i} \text{L}_{\lambda} (\loss_i, \sigma_i)
\\
 \text{SL}_\lambda(\loss_i) &= \text{L}_\lambda(\loss_i, \sigma^{*}_{\lambda}(\loss_i, \sigma_i)) = \min_{\sigma_i} \text{L}_\lambda (\loss_i, \sigma_i),
\end{split}
\end{align}

Using this technique, the confidence parameters are not required to be learned during the training. \citet{Castells2020SuperLossAG} found out that $\sigma^{*}_{\lambda} (\loss_i)$ has a closed-form solution, computed as follows,


\begin{equation}
     \sigma^{*}_{\lambda} (\loss_i) = e ^ {-W (\frac{1}{2} \max (-\frac{2}{e}, \beta))}, \beta = \frac{\loss_i - \tau}{\lambda}
\end{equation}
in which $W$ is the Lambert W function. With this in mind, \superl{} upweights easier samples dynamically during the training, providing a curriculum learning approach to summarization. We call this model \currsum{} in our experiments. 
% We also experiment with a combination of \sentsum{} and \currsum{} models and name it \currsentsum{} throughout our experiments.



==> SECTIONS/04_experimental.tex <==








\section{Experimental Setup}
\label{sec:res}
% In this section, we describe the datasets, baseline models, and model implementation.

\subsection{Dataset}
We use the \mentsum dataset in our experiments. This dataset contains over 24k post-\tldr{} pairs, making up 21,695 (train), 1209 (validation), and 1215 (test) instances, and is gathered by mining 43 mental health subreddit communities on Reddit with rigorous filtering rules. We refer the readers to the main paper for more details on this dataset~\cite*{Sotudeh2022MentSumAR}. 
% It is worth noting that Reddit TIFU split was suggested by \citet{zhang2019pegasus}.

\subsection{Comparison}
We compare our model against the \bart{}~\cite{Lewis2020BARTDS} baseline, which does not utilize the curriculum learning objective. \bart is an abstractive model that uses a pre-trained encoder-decoder architecture, unlike \textsc{Bert} which only utilizes a pre-trained encoder. As shown in \cite*{Sotudeh2022MentSumAR}, \bart{} is the strongest baseline; thus, we apply CL on it to evaluate its impact on summarization. We refer the reader to the original paper for more extractive and abstractive baselines.

% \noindent \textsc{\textbf{LexRank}}~\cite{Erkan2004LexRankGL}: an unsupervised extractive summarization method that uses graph-based centrality techniques to score source sentences.

% \begin{itemize}[leftmargin=*,label={-}]
% \item \textsc{\textbf{Lead-2}}: a simple extractive baseline that picks two first sentences of user's post as the summary. 

% \item \textsc{\textbf{LSA}}~\cite{Steinberger2004LSA}: a non-neural extractive baseline that employs the Singular Value Decomposition (SVD) for finding hidden semantic structures between words and sentences. 

% \item \textsc{\textbf{LexRank}}~\cite{Erkan2004LexRankGL}: a non-neural unsupervised extractive model that uses graph centrality model for detecting the most salient sentences and concatenate them to form the final extractive summary. 


% \item \textsc{\textbf{BertSumExt}}~\cite{Liu2019TextSW}: the extractive variant of \textsc{BertSum} that inserts external \texttt{[CLS]} tokens between sentences. The representations are further used with a Sigmoid classifier to compute sentence extraction probabilities.

% \item \textsc{\textbf{BertSumAbs}}~\cite{Liu2019TextSW}: the abstractive variant of \textsc{BertSum} that uses a Transformer-based encoder-decoder architecture. The encoder is \textsc{Bert}, but decoder is pre-trained from scratch. 

% \item \textsc{\textbf{BertSumExtAbs}}~\cite{Liu2019TextSW}: a two-stage fine-tuning approach, for which \textsc{BertSumExtAbs} first fine-tunes encoder on extractive summarization, then it is fine-tuned along with decoder for abstractive summarization task. 

% \item \textsc{\textbf{MatchSum}}~\cite{zhong-etal-2020-extractive}: an extractive framework which matches source text with candidate summaries in a semantic space. Unlike commonly used extractive summarizers, \textsc{MatchSum} does not rely on extracting sentences individually, instead it selects a set of sentences (i.e., candidate summary) that has the maximum semantic similarity with the ground-truth summary. 


% \noindent \textsc{\textbf{Pegasus}}~\cite{zhang2019pegasus}: an abstractive  model that defines a new pre-training task as Gap Sentence Generation (GSG), in which key source sentences are masked out, and the network learns to generate the missing sentences.
% \textsc{

% \end{itemize}
% \noindent \textsc{\textbf{NeuTopicSumm}}~\cite{Nguyen2021EnrichingAC}: an abstractive baseline that incorporates neural topic model into summarization framework.

% \noindent \textsc{\textbf{BART+R3F}}~\cite{Aghajanyan2021BetterFB}: a summarization method that proposes a new fine-tuning technique; R3F method replaces previously proposed adversarial objectives with parametric noise, and discourages representation change during fine-tuning without degrading the performance. 

% \noindent \textsc{\textbf{BART+MUPPET}}~\cite{Aghajanyan2021MuppetMM}: an architecture that introduces an additional large-scale learning stage (i.e., pre-finetuning) between the pre-training and fine-tuning stages, using a large-scale collection of datasets proposed on different tasks. \textsc{MUPPET} is designed to encourage representation learning for increasing the generalization of language models.


\subsection{Implementation details}
We use the Huggingface's Transformers library ~\cite{Wolf2020Transformers}~\footnote{\url{https://github.com/huggingface/transformers}} to implement our models.
% , and make the code publicly available to expedite future research~\footnote{\textit{HTTP}}. 
We train all of our models for 8 epochs, performing evaluation step in intervals of 0.5 epochs, and use the checkpoint that achieves the best \textsc{Rouge-L} score in the validation for the inference. 
% The validation is performed every 1k (Reddit TIFU) and 2.5k (Webis-TLDR-17) training steps. 
AdamW optimizer~\cite{Loshchilov2019DecoupledWD} initialized with learning rate of $3e-5$, $(\beta_1, \beta_2)= (0.9, 0.98)$, and weight decay of 0.01 is used for all of our summarization models, as well as for \textsc{Bart}. 
% Specifically, to train \sentsum{}, we use a lower learning rate of $1e-5$ for the pre-trained part. 
Cross-entropy loss is used for all models. 
% except for pre-training \sentsum{} where we use the Mean Squared Error (MSE) loss function. 
% For \textsc{BertSum} variants, we use the main code-base~\footnote{\url{https://github.com/nlpyang/PreSumm}} and default hyper-parameters suggested by the original paper~\cite{Liu2019TextSW}. 
To keep track of the learning process, we use Weights \& Biases~\cite{wandb} toolkit~\footnote{\url{https://wandb.ai/}}. 
% We employ 5 human evaluators familiar with data science and annotation through the Upwork~\footnote{\url{https://www.upwork.com}} freelancing platform, each paid 200USD for performing independent evaluation on provided samples.

\section{Ethics and privacy}
While we use publicly available Reddit data to train and validate our model, we recognize that special care should be taken when dealing with this type of data due to its sensitivity and users' privacy~\cite{Benton2017EthicalRP,Nicholas2020EthicsAP}. Thus, we have made no attempts to identify, contact the users, or explore user relations to trace their social media account. It has to be mentioned that the \mentsum{} dataset is distributed through Data Usage Agreement (DUA)~\footnote{\url{https://ir.cs.georgetown.edu/resources/mentsum.html}} document to further ensure that users' identity would never be disclosed.
% while conducting research on mental health summarization task. 

==> SECTIONS/05_results.tex <==


\begin{table}[t]
\centering
\scalebox{0.8}{
 
   \begin{tabular}{l@{\hspace{1.1cm}}rrrr}
       \toprule
           
     Model                    & {R-1}  & {R-2}  & {R-L} & {BS} \\
    \midrule
    % \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize	 Extractive}}} 
    % & LexRank \cite{Erkan2004LexRankGL}                 &  & 18.87 & 8.48 & 17.72 \\
    %  \textsc{LexRank}~\cite{Erkan2004LexRankGL}                        & - & - & - \\
       \textsc{OracleExt}             &  35.98 & 11.59 & 23.21 & 82.72 \\
    %  \textsc{Lead-2}             &  20.09 & 3.57 & 13.70 \\

    %  \vspace{0.3em} \\
    % \hdashline[0.5pt/2pt] \vspace{-0.8em} \\
    % \multirow{4}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize Abstractive}}} 
    %       \textsc{LSA}~\citeyearpar{Steinberger2004LSA}             &  22.96 & 3.98 & 14.50 \\
    %  \textsc{LexRank}~\citeyearpar{Erkan2004LexRankGL}    & 23.21     & 4.42     & 15.19     \\
    %      \textsc{BertSumExt}~\citeyearpar{Liu2019TextSW}                             & 26.64 & 5.83 & 16.66 \\
                %   \textsc{MatchSum}~\cite{zhong-etal-2020-extractive}                             & 26.29 & 6.32 & 17.12 \\


    %  \textsc{BertSumAbs}~\citeyearpar{Liu2019TextSW}                             & 25.35 & 6.49 & 17.11 \\
    %  \textsc{BertSumExtAbs}~\citeyearpar{Liu2019TextSW}                 & 25.75 & 6.80 & 17.48 \\

     
     \textsc{Bart}~\citeyearpar{Lewis2020BARTDS} & 29.13 & 7.98 & 20.27 & 85.01  \\
     
    \hdashline[2pt/2pt] \vspace{-0.8em} \\
    \currsum{} (Ours) & \textbf{30.16}& \textbf{8.82}& \textbf{21.24} & \textbf{86.32} \\
    \bottomrule  
\end{tabular}
    
    
}
    

\caption{\textsc{Rouge} and \textsc{Bertscore} results on test set of \mentsum dataset. As \bart{} was the most performant baseline provided in ~\cite*{Sotudeh2022MentSumAR}, we evaluate the effectiveness of Curriculum on \bart in this work. For other baselines, we refer the reader to the main paper.
}
\label{tab:final}
\vspace{-1em}

\end{table}
\section{Results}
% In this section, we first provide the experimental results of the baselines models and compare them with our models' performance. Following experimental results, we then describe the details of the extensive human evaluation carried out to provide insights into the qualities of our model against the best perfoming baseline. 
\begin{table*}[t]
\centering\small
% \def\arraystretch{2.5}
\scalebox{.8}{
\begin{tabular}{ p{0.3\linewidth}  p{0.4\linewidth}  p{0.4\linewidth}}
\toprule
       Human-written & \bart-generated & \currsum-generated \\ \midrule
      
    %   \footnotesize \textit{Me xxx and my wife xxx are thinking of having a child within the next year. Aside from having anxiety about the state of the world and passing on my ADHD I cannot shake the feeling that I won't be attentive enough to the child or I will lose interest in being a father like I do with so many other things in my life. The last thing I want is to be a shi**y dad, so party of me thinks it's better to not take the chance and just never have a child. What do you guys think? Also if any ADHD parents have any input please let me know how your experience has been.} 
      
    %   &
     \vspace{.25em}
      \textit{... having kids ... my ADHD ...  opinions on parenthood...} 

      & 
          \vspace{.25em}

      \footnotesize \textit{I think it's better to \textcolor{gray}{not have a child} now than \textcolor{gray}{never having a child} in the future.}
      
      &
          \vspace{.25em}

      \textit{I'm \textbf{thinking of having a child} and I \textbf{ don't want to be a shi**y dad} for my \textbf{ADHD}. Any \textbf{parents with ADHD experience?}}
          \vspace{.25em}

      \\
      
      \midrule
      
    %   \textit{I think I am clinically depressed xxx. Maybe it's SAD, because I begin to feel worse in mid-November, February is absolute shi**, and I am only starting to a bit feel better now this could also be because I am busy preparing to move. I live in xxx state. I have pretty much every symptom on this list. }
      
    %   &
          \vspace{.25em}

      \textit{... symptoms of depression ... go to get help ...}
      
      &
          \vspace{.25em}

      \textit{I think I \textbf{am clinically depressed}, and I have pretty much \textbf{all the symptoms of depression}, so I am \textcolor{gray}{asking for help}}
      
      &
          \vspace{.25em}

      \textit{I think I am \textbf{clinically depressed} xxx. I have pretty much \textbf{every symptom on this list}.}   %%%%%%
          \vspace{1.5em}

      
      \\
      
      \midrule
      \vspace{.25em}
      \textit{... free of anxiety for a decade.. symptoms come ... }
      
      &
      
      \vspace{.25em}
      \textit{I've been \textbf{free of anxiety} \textcolor{gray}{for less than a week} and I'm afraid that it's only a temporary solution. \textcolor{gray}{I don't know what to do.}}
      
      &
      \vspace{.25em}
      \textit{I've been \textbf{free of anxiety for a decade} and I'm afraid that if the \textbf{symptoms start to come back}, I'll be able to \textbf{slip back into it} again.}
      
      \vspace{1.25em}
      
      
      \\
      \midrule
      
    %   \footnotesize\textit{I really like her. I spent most of my day with her today because she was training me on the cash register. I was really awkward at first, but an hour or two later she kinda started breaking the ice, asking basic questions like "Do you have any brothers or sisters?" that sparked into mini conversations, but I don't recall really asking her anything not work related the whole time beside when she would bring something up first. Most of your time was spent in awkward silence up until the last half hr of four hours. I was pretty nervous. I'm xxx and she's xxx going on xxx. I like her and I want to get to a place where I can ask her out, but I don't want to ruin that chance in the process. Some possibly useful info I am new to this town and don't know anyone outside of family yet.}
      
    %   &
      \vspace{.25em}
      \textit{... ask her out ... barely talked to her... mess up my chance...}
      
      &
      \vspace{.25em}
      \textit{I like a girl \textcolor{black}{at work} and I want to \textbf{ask her out}, but I don't want to \textbf{ruin that chance} in the process.}
      
      &
      \vspace{.25em}
      \textit{I like a girl at work, but \textcolor{gray}{I don't know how to \textbf{ask her out.}}}
        \vspace{1.5em}
        \\      
      \bottomrule
      
      
    \end{tabular}
}
\caption{Four samples of the the human-written, \bart{}-generated, and \currsum-generated \tldr{} summaries. The human-written samples are partially shown to preserve users' privacy. That is, we have only shown the important human-written phrases to trace them within the generated summaries. The text that is unfaithful to the post (i.e., not supported by the user post) is in \textcolor{gray}{Gray} and the salient information that is picked up by the summarization systems is shown in \textbf{Bold}.}
\vspace{-1em}
\label{tab:er}
\end{table*}
\textbf{Automatic evaluation.}
Table \ref{tab:final} reports the performance of the baseline model along with our model's in terms of \textsc{Rouge} score variants~\cite{Lin2004ROUGEAP} and \textsc{Bertscore}~\cite{Zhang2020BertScore} over \mentsum dataset. As indicated, the best model is our \currsum{} that uses \superl{} curriculum directly on top of the \bart{} model and is a clear improvement over it across all metrics, achieving the current state-of-the-art performance. 
Specifically, our model outperforms its ground baseline that has no curriculum (i.e., \bart{}) by  improvement gains of 3.5\%, 10.4\%, 4.7\%, 1.5\% for \rgo, \rgt, \rgl, \textsc{bertscore},  respectively. Having looked at the \textsc{OracleExt} scores which shows the upper bound performance of an ideal extractive summarizer, it seems that there is room for improvement on the extractive setting to achieve state-of-the-art performance. More sophisticated models can invest in extractive or hybrid summarization models such as those done in ~\cite{Gehrmann2018BottomUpAS, MacAvaney2019SIG,Sotudeh2020AttendTM}. 

% 12.6\%, 1.8\% (\rgt); 5.4\%, 4.4\% (\rgl) 
% on \mentsum. 
% While \currsum{} achieves competitive performance in terms of \rgo{} with \textsc{BART+R3F} and \textsc{BART+MUPPET}, it lags behind them on \rgt{} and \rgl. These differences may be explained by the fact that \textsc{BART+R3F} is computationally more intensive than our curriculum-based model~\footnote{BART+R3F adds an additional forward pass (FP) to compute symmetric KL divergence term for measuring parametric noise.}, and \textsc{BART+MUPPET} performs the best presumably due to its additional large-scale learning stage (i.e., pre-finetuning) that is not considered in \bart{} and \currsum~\footnote{BART+MUPPET is not released at the time of writing this study; hence, we could not report its performance when curriculum is applied.}.
% Interestingly, while augmenting the decoder with sentence cross-attention module (i.e., \sentsum) is marginally better than the \bart{} baseline, training it with curriculum learning \superl{} function (i.e., \currsentsum) further improves the performance. This finding provides a compelling evidence for the usefulness of curricular training strategy applied in summarization task. Comparing abstractive vs. extractive models, we observe a noticeable performance gap denoting that Reddit TIFU includes rather abstractive summaries than extractive. 



% Comparing the extractive baselines vs. our abstractive model, it is observed that our model significantly outperforms the extractive models indicating the strong abstractiveness characteristic of the \mentsum dataset. Although, looking at \textsc{OracleExt} ---which shows the upper bound performance of the extractive systems, it appears that the more sophisticated extractive systems can close this gap, which is left for future work. 





\noindent \textbf{Case study and analysis.}
While our proposed model significantly improves upon the \bart{} baseline, we recognize the limitations of \textsc{rouge} metric in evaluation of summarization systems~\cite{Cohan2016RevisitingSE}. In order to explore the qualities and limitations of our work, we analyze the human-written \tldr{}s along with the generated results by \bart and our model, comparing them against each other. Table \ref{tab:er} shows four samples of the human and systems generated \tldr{}s. As seen, our model can improve the faithfulness of the summary~\footnote{Faithfulness is defined as generating output text that is supported by the user post.} in the first, second, and third samples. Having looked at other cases in our study, it appears that curriculum learning positively mitigates faithfulness errors. This might be attributed to the fact that the summarizer can achieve an improved \textit{understanding} of the source document when the contribution of each sample is controlled in each iteration of the learning process. Looking at the second sample, it turns out that our model can improve the conciseness of the summaries; that is, briefly conveying the main points within the summary. Comparing system-generated summaries in the fourth sample, it is observed that our system generated a phrase (shown in Gray) by mixing up different regions of the user post. Surprisingly, it appears that ``\textit{I don't know how/what to}'' is a common phrase used in most human-written summaries that are seeking advice from the community. The experimented summarization systems (i.e., \bart{} and ours) adhere to overgenerating this phrase. 

% It is also notable that \textsc{BertSumExtAbs} model could improve upon both extractive and abstractive variants of the \textsc{BertSum} model. This is in agreement with our hypothesis that making abstractive summarizer aware of sentential saliency is effective at producing final summary, although incorporation of sentence attention to decoder (i.e., \sentsum) could slightly improve upon its \bart{} ground.

% Unexpectedly, no significant difference is observed when adding sentence self-attention to decoder (i.e., \sentsum{} model) compared to the \bart{} model. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.3]{FIGS/val_peformance.pdf}
%     \caption{Comparison of our models' performance vs. \bart's on validation set in terms of \textsc{Rouge-L} score.}
%     \label{fig:val_performance}
% \end{figure}

% \begin{figure}[t]

%     \begin{tabular}{ll}
%     \hspace{-0.7cm}
%     \includegraphics[scale=0.205]{FIGS/val_peformance_1.pdf}
    
%     &
%     \hspace{-0.5cm}
%     \includegraphics[scale=0.205]{FIGS/val_peformance_2.pdf}
    
    
%     \end{tabular}
    
%     % \includegraphics{}
%     \caption{Plots demonstrating the validation performance of various models with increasing steps of training of Reddit TIFU dataset. Blue lines show the performance when no curriculum is used. Red lines represent the performance when the curriculum is added. Vertical lines indicate the step where the models achieve the \rgl{} score that the baselines attain at convergence.}
%     \label{fig:val_performance}
%     \vspace{-0.3cm}
% \end{figure}


% We further investigate the validation performance of the summarization models in the presence and absence of the curriculum learning strategy. As shown in Figure \ref{fig:val_performance}, models trained with curriculum strategy (i.e., \currsum{} and \currsentsum) tend to converge faster, and perform better in comparison with their respective baselines (i.e., \bart{} and \sentsum) that are without curriculum learning. 
% Specifically, \sentsum{} starts with quite a low \rgl{} score compared to the other models, although as training continues, it attains better scores on the next validation steps. 
% This discrepancy at the early stages of training might be due to the fact that \sentsum's weights are initialized with the fine-tuned model from a different task (i.e., sequence tagging problem), and abstractive summarizer has difficulty at fine-tuning it on early training stages. 
% Looking at Figure \ref{fig:val_performance}, the efficiency of curriculum strategy is quite remarkable considering the scores and convergence steps (i.e., vertical red lines) of the curriculum-equipped models.

% This supports the hypothesis on curriculum learning strategy that noted faster convergence and reduced training time as a result of employing this strategy. 
% For instance, comparing \sentsum{} with \currsentsum{}, we see that the summarizer attains top validation scores in first training stages; hence, faster convergence.
% Interestingly, the improvement gap is even larger for our models (compared to \bart{}) when evaluated on the test set. This seconds the evidence that curricular learners help generalizing training patterns efficiently to unseen data. 

% \noindent\textbf{What is the effect of curriculum learning on cross-domain datasets? } To measure the cross-domain performance of models supplied with curriculum learning strategy, we compare \bart's performance (as a transformer-based  state-of-the-art summarizer) vs. a variant of \bart{} with curriculum strategy (i.e., our \currsum{} model) on three summarization datasets: Webis-TLDR-17, CNN/DM, and XSum. Results, summarized in Table \ref{tab:tab2}, are a strong indication of effectiveness of curriculum learning on datasets from various domains (i.e., Social Media and News) as we observe a consistent improvement compared to the \bart{} baseline.


% \begin{figure*}[t]
% \centering
% \bgroup
% \setlength{\tabcolsep}{0pt}
% \renewcommand{\arraystretch}{0}
% \begin{tabular}{cccccc}
% \includegraphics[scale=0.15]{FIGS/arrow_figs//Ours-Human-fluency-5.pdf} &
% \includegraphics[scale=0.15]{FIGS/arrow_figs//Ours-Human-info-5.pdf} &
% \includegraphics[scale=0.15]{FIGS/arrow_figs//Ours-Human-quality-5.pdf} &
% \includegraphics[scale=0.15]{FIGS/arrow_figs//Ours-Bart-fluency-5.pdf} &
% \includegraphics[scale=0.15]{FIGS/arrow_figs//Ours-Bart-info-5.pdf} &
% \includegraphics[scale=0.15]{FIGS/arrow_figs/Ours-Bart-quality-5.pdf} \\
% (a) & (b) & (c) & (d) & (e) & (f) \\
% \end{tabular}
% \vspace{-0.5em}
% \caption{Histograms and arrow plots depicting score transition between 200 manually-scored \tldr{} summaries. (a--c) and (d--f) show our system's comparison with human and \bart{} baseline system, respectively. Although comparable in terms of fluency metric with the baseline and human parity, our model makes a strong gain to improve summary's informativeness and overall quality.}
% \label{fig:arrows}
% \egroup
% \end{figure*}

% \begin{table}[t]
%     \centering
% \scalebox{0.8}{
% \begin{tabular}{c}
    
%   \begin{tabular}{l@{\hspace{1.2cm}}lll}
%     \toprule
%      Model                    & \textsc{RG-1}  & \textsc{RG-2}  & \textsc{RG-L}  \\
%          \midrule
%     \textsc{Bart}~\cite{Lewis2020BARTDS}  &  20.73 &  6.79 & 17.22 \\
     
%     \currsum{} (Ours)  & \textbf{22.12}& \textbf{6.91} &  \textbf{17.97} \\
    
%     \bottomrule 
%     % \vspace{-0.8em} \\ 
%     \end{tabular}
    
%         \vspace{0.1cm} \\
%          (a) Webis-TLDR-17 \vspace{0.2cm} \\
          
%   \begin{tabular}{l@{\hspace{1.2cm}}lll}
%     \toprule
%      Model                    & \textsc{RG-1}  & \textsc{RG-2}  & \textsc{RG-L}  \\
%          \midrule
%     \textsc{Bart}~\cite{Lewis2020BARTDS}  &  44.16 &  21.28 & 40.90 \\
     
%     \currsum{} (Ours)  & \textbf{44.49}& \textbf{21.53} &  \textbf{41.19} \\
    
%     % \vspace{0.2cm} \\
%         %  (b) \vspace{0.4cm} \\
    
%     \bottomrule 
%     % \vspace{-0.8em} \\ 
    
%     \end{tabular}
    
%     \vspace{0.1cm} \\
%          (b) CNN/DM \vspace{0.2cm} \\
    
%     \begin{tabular}{l@{\hspace{1.2cm}}lll}
%     \toprule
%      Model                    & \textsc{RG-1}  & \textsc{RG-2}  & \textsc{RG-L}  \\
%          \midrule
%     \textsc{Bart}~\cite{Lewis2020BARTDS} &  45.14 &  22.27 & 37.25 \\
     
%     \currsum{} (Ours)  & \textbf{45.41}& \textbf{22.39} &  \textbf{37.41} \\
    
%     \bottomrule  
    
%     % \vspace{-0.8em} \\ 
%     \end{tabular}
%       \vspace{0.1cm} \\
%          (c) XSum  
%     \end{tabular}
    
% }
    
    
    
%     \caption{Results when applying curriculum learning for \bart{} on cross-domain datasets. }
%     \label{tab:tab2}
% \vspace{-0.4cm}
% \end{table}

% \noindent \textbf{Human evaluation.}
% A few studies have recognized the limitation of widely adopted \textsc{Rouge} metric as it is biased toward surface lexical similarities~\cite{Ng2015BetterSE, Cohan2016RevisitingSE}. To get insights into the qualities of our proposed models, we performed a human evaluation over a random set of system-generated summaries. To this end, we randomly sampled 200 cases from Reddit TIFU's test set, each consisting of the post's source text along with blinded \tldr's from (1) author-written references; (2)  \bart{} baseline; and (3) our \currsentsum{} model. The choice of \currsentsum{} lies in the fact that we want to evaluate the effect of both sentence attention and curriculum learning in our human evaluation process. To prevent potential bias, we randomly shuffled the ordering of \tldr s provided to evaluators. Following prior work~\cite{Grusky2018NewsroomAD, Zhang2020OptimizingTF, Cho2021StreamHoverLT}, we define three metrics: (1) \textbf{Fluency: } is the \tldr{} well-written and easy to understand? (2) \textbf{Informativeness: } does the \tldr{} provide useful information about source? (3) \textbf{Overall quality: } overall, is the \tldr{} of good quality in terms of content (both fluency and informativeness), and correctness?  We then had five human evaluators score each of the provided examples on a scale of [1-5] (worst to best) in terms of the criteria mentioned above. The evaluators were familiar with data science and annotation and were hired through the Upwork~\footnote{\url{https://www.upwork.com}} freelancing platform.


% \begin{table}[t]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lccc}
%         \toprule
%          System & Fluency & Info. & Overall  \\
%          \midrule
%          \bart{} & 4.48 & 3.76 & 3.75   \\
%          \currsentsum & 4.45 & \textbf{3.91} & \textbf{3.98}  \vspace{0.25em} \\ 
%           \hdashline[0.5pt/2pt] \vspace{-0.85em} \\ Human & \textbf{4.50} & 3.72  &  3.70 \\ 
%          \bottomrule
%     \end{tabular}
%     }
%     \caption{Results of the human evaluation comparing three systems in terms of {Fluency}, {Informativeness}, and {Overall quality}. Winning scores are shown in bold.}
%     \label{tab:human_evaluation}
%     % \vspace{-0.5em}
% \end{table}




% Table \ref{tab:human_evaluation} shows the average score gained by each system in terms of the aforementioned qualitative criteria. Comparing our model against other systems, we find that: (1) in terms of fluency, our model and \bart{} are quite comparable, with human summaries being the best; (2) we calculated the average \tldr{} length (in tokens) of the test set and obtained 22.9 (Human), 23.6 (\bart), and 19.8 (\currsentsum). Interestingly, despite generating shorter summaries, our model outperforms both \bart{} and human-written \tldr s on informativeness which shows that it efficiently selects the useful information from the original text, generating them in a comparably shorter text. Looking into the outperformed cases on informativeness, we noticed that the annotators tend to give a higher score to a summary if it provides the most important information within a concise text (i.e., providing only to the point information akin to the definition of \tldr), which is generally achieved by our model.
% % We observed that while our model generates shorter \tldr s, it still covers more useful information within the generated shorter \tldr s as compared to Human and \bart -generated ones; 
% (3) our model is also more preferable in terms of overall quality compared to \bart{} and human summaries, with relatively large gap. Overall, it is interesting that summarization models are becoming comparable (sometimes even more preferable) to Human \tldr s on informativeness and overall quality, substantiating the recent success of pre-trained language models as also shown by~\citet{Fabbri2021SummEvalRS}. We further computed the Fleiss' Kappa~\cite{Fleiss1971MeasuringNS} inter-rater agreement for the qualitative metrics, and obtained 10\%, 27\%, 22\% correlation scores for fluency, informativeness, and overall quality, respectively. These correlations are considered to be ``slight'' for fluency and ``fair'' for informativeness, and overall quality with regard to the Fleiss' range interpretation~\cite{Landis1977TheMO}. Table~\ref{tab:agreement} shows the system-wise Fleiss' agreement over three metrics, expressing that agreement rates on our system summaries are stronger than the others.

% \begin{table}[t]
%     \centering
%         \scalebox{0.85}{
%     \begin{tabular}{lccc}
%          \toprule
%          System & Fluency & Info. & Overall  \\
%          \midrule
%          \bart{} & 12\% & 26\% & 21\% \\
%          \currsentsum & \textbf{14\%} & \textbf{33\%} & \textbf{25\%} \\
%          Human & 11\% & 24\% & 20\% \\
%          \bottomrule
%     \end{tabular}
%     }
    
%     \caption{System-wise Fleiss' kappa agreement}
%         \vspace{-0.5em}

%     \label{tab:agreement}
% \end{table}


% Inspired by ~\citet{MacAvaney2019SIG, Sotudeh2020AttendTM}, we plot histograms and arrow plots for our human evaluation in Figure \ref{fig:arrows}. The histograms show the score distributions gained by each model, and arrow plots demonstrate the score transition (i.e., how scores changed) on the provided samples. The head of each arrow shows our system's score, which makes a transition to its head showing the score gained by the other systems (either human or \bart). The count of the samples that have made a specific score transition is shown next to the arrows' tail.  As indicated, it is observable that our system makes a strong gain in informativeness and overall quality metrics over the other two systems while staying competitive in terms of fluency. The improvement is specifically considerable in enhancing scores from 4 to 5 in informativeness and overall quality metrics.

% \noindent \textbf{Qualitative analysis.}
% In order to provide insights into qualities of our model vs baselines, we did further evaluation over the annotated samples. We found out that (1) our model performs superior at collecting the key information from the source when there is an overload of important information in the source text, while most gold \tldr s contain just a few sentences (less than 3) that only include the most important information. This behaviour of our model enables it to take advantage of informativeness and overall quality metrics. (2) human-written \tldr s receive relatively a lower score compared to our model's in terms of informativeness and overall quality when the human-written \tldr{} contains entailment/conclusion from the source, although it might not be present in the source text. (3) interestingly, as the system \tldr s become lengthy, the annotators tend to give a lower score in terms of informativeness and overall quality metrics. This might be due to the fact that longer summaries encompass a high proportion of source information regardless of their saliency. 
% (4)  human \tldr s are written informally with truncated style, while our system-generated \tldr s are complete sentences that improve fluency. 
% Considering these errors made by our system, we believe that future work can continue the work on this direction by developing models that incorporates text entailment into the summarizer. 

==> SECTIONS/06_conc.tex <==
\section{Conclusion}
Generating short summaries given the users' online posts can save counselors' reading time, and reduce their fatigue. On this basis, they can provide faster responses to community users. While neural Transformers-based summarization models have shown to be promising, they suffer from \textit{inefficient training process} that hinders their potentials for showing a promising performance. To compensate for this issue, in this paper, 
%  Firstly, 
%  we propose to tackle the content selection problem by augmenting the decoder via a sentence cross-attention layer such that the decoder becomes aware of sentence saliency. Secondly,
we incorporated a confidence-aware curriculum learning  approach, which uses task-agnostic \textsc{SuperLoss}, to the summarization framework in the hope of increasing model's generalization, and ultimately improving model performance. Our automatic evaluations over \mentsum dataset of mental health posts show the effectiveness of our model, yielding 3.5\%, 10.4\%, 4.7\%, 1.5\% relative improvements over \bart{} summarizer on \rgo, \rgt, \rgl, and \textsc{bertscore}, respectively. Our model tailors the new state-of-the-art performance on \mentsum{} dataset. We further showed various system-generated summaries to showcase the qualities and limitations of our proposed model. 
